Learning to Retrieve Passages without Supervision

Dense retrievers for open-domain question answering (ODQA) have been shown to achieve impressive performance by training on large datasets of question-passage pairs. In this work we ask whether this dependence on labeled data can be reduced via unsupervised pretraining that is geared towards ODQA. We show this is in fact possible, via a novel pretraining scheme designed for retrieval. Our "recurring span retrieval" approach uses recurring spans across passages in a document to create pseudo examples for contrastive learning. Our pretraining scheme directly controls for term overlap across pseudo queries and relevant passages, thus allowing to model both lexical and semantic relations between them. The resulting model, named Spider, performs surprisingly well without any labeled training examples on a wide range of ODQA datasets. Specifically, it significantly outperforms all other pretrained baselines in a zero-shot setting, and is competitive with BM25, a strong sparse baseline. Moreover, a hybrid retriever over Spider and BM25 improves over both, and is often competitive with DPR models, which are trained on tens of thousands of examples. Last, notable gains are observed when using Spider as an initialization for supervised training.

==> table_e2e_unsup.tex <==
% \begin{table}[t!]
% \small
% \centering
% \begin{tabular}{lccc}
% \toprule
% \multirow{2}{55pt}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{NQ}} & \textbf{TQA} \\
% & \textbf{Dev} & \textbf{Test} & \textbf{Test}\\
% \midrule
% ICT \cite{sachan-etal-2021-end,sachan2021emdr} & 28.0 & 32.3 & 40.2 \\
% REALM \cite{Guu2020REALMRL} & 38.5 & - & - \\
% MSS \cite{sachan-etal-2021-end} & - & 41.7 & 53.3 \\
% MSS$^2$ \cite{sachan2021emdr} & 38.6 & - & - \\
% \textbf{\ourmodel} & 46.5 & 49.6 & 63.6 \\
% \textbf{\ourmodel~+ BM25} & \textbf{53.3} & \textbf{55.1} & \textbf{71.7} \\
% \bottomrule
% \end{tabular}
% \caption{Top-5 retrieval accuracy of unsupervised retrievers on Natural Questions and TriviaQA. REALM, MSS and MSS$^2$ (stands for MSS-EMDR$^2$) are initialized with a pretrained ICT model and are trained end-to-end, jointly with a reader.}
% \label{tab:unsup_e2e}
% \end{table}

==> table_no_overlap.tex <==
% \begin{table}[t!]
% \small
% \centering
% \begin{tabular}{lccc}
% \toprule
% \textbf{Model} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{WQ} \\
% \midrule
% DPR-Single & \textbf{76.8} & 62.6 & \textbf{71.1} \\
% DPR-Multi  & \textbf{77.1} & 62.4 & 70.4 \\
% \midrule
% BM25 & 70.1 & 62.4 & 66.4 \\
% ICT & 51.3 & 14.2 & 52.1 \\
% Condenser & 26.6 & ~~9.1 & 30.8 \\
% CoCondenser & 52.4 & 13.8 & 54.2 \\
% \ourmodel~(Ours) & 71.7 & 61.4 & 68.9 \\
% BM25 + \ourmodel~(Ours) & \textbf{76.6} & \textbf{64.1} & \textbf{71.6} \\
% \bottomrule
% \end{tabular}
% \caption{Top-100 retrieval accuracy on the ``\textit{no answer overlap}'' portion of the test sets \cite{lewis-etal-2021-question}. Only questions with answers that are not present in the training data of the corresponding dataset are kept. DPR-Single is trained on the corresponding dataset only. Results with up to a 0.5-point difference from the best are marked in bold. }
% \label{tab:overlap}
% \end{table}


% \begin{table}[t!]
% \small
% \centering
% \begin{tabular}{lccc}
% \toprule
% \textbf{Model} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{WQ} \\
% \midrule
% DPR-Single & 68.7 & 56.4 & 60.0 \\
% DPR-Multi  & 68.8 & 55.8 & 60.5 \\
% \midrule
% BM25 & 55.5 & 56.0 & 53.6 \\
% ICT & 33.5 & ~~7.0 & 32.0 \\
% Condenser & 13.3 & ~~4.2 & 19.3 \\
% CoCondenser & 36.8 & ~~8.0 & 38.3 \\
% \ourmodel~(Ours) & 57.3 & 53.4 & 53.0 \\
% BM25 + \ourmodel~(Ours) & 64.8 & 58.6 & 59.1 \\
% \bottomrule
% \end{tabular}
% \caption{Top-20 retrieval accuracy on the ``\textit{no answer overlap}'' portion of the test sets \cite{lewis-etal-2021-question}. Only questions with answers that are not present in the training data of the corresponding dataset are kept. DPR-Single is trained on the corresponding dataset only.}
% \label{tab:overlap}
% \end{table}

==> table_original_test_sets.tex <==
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{cllcc|cc|cc}
% \toprule
%  & \multirow{2}{55pt}{Model} & \multirow{2}{30pt}{Mode} & \multicolumn{2}{c|}{\textbf{NQ}} & \multicolumn{2}{c|}{\textbf{TriviaQA}} & \multicolumn{2}{c}{\textbf{WQ}}  \vspace{0.5pt} \\
%  &  &  & \textbf{Top-20} & \textbf{Top-100} & \textbf{Top-20} & \textbf{Top-100} & \textbf{Top-20} & \textbf{Top-100}  \\
% % \midrule
% % \textit{Supervised Methods} & & & & & & &  \\
% \midrule
% \multirow{4.3}{55pt}{\textbf{\textit{Supervised}}} & DPR-Single & Dense  & 80.1 & 86.1 & 79.7 & 85.1 & 74.3 & 82.2 \\
% & DPR-Multi & Dense & 79.5 & 86.1 & 78.9 & 84.8 & 75.1 & 83.0  \\
% \cmidrule{2-9}
% & DPR-Single + BM25 & Hybrid & 82.9 & 88.3 & 82.4 & 86.5 & 75.1 & 83.1 \\
% & DPR-Mutli + BM25 & Hybrid & 82.6 & 88.2 & 82.6 & 86.5 & 77.2 & 84.5 \\
% \midrule
% % \textit{Unsupervised Methods} & & & & & & &  \\
% % \midrule
% \multirow{7}{55pt}{\textbf{\textit{Unsupervised}}}&BM25 & Sparse & 62.9 & 78.3 & 76.4 & 83.2 & 62.4 & 75.5 \\
% \cmidrule{2-9}
% &ICT  & Dense & 50.6 & 66.8 & 57.5 & 73.6 & 43.4 & 65.7 \\
% & Condenser & Dense &  25.5 & 43.4 & ~~9.6 & 18.5 & 35.8 & 51.9 \\
% & CoCondenser & Dense & 46.8 & 63.5 & 13.8 & 24.3 &  50.7 & 68.7 \\
% &\textbf{\ourmodel} & Dense & 65.9 & 79.8 & 74.2 & 82.9 & 65.3 & 79.7 \\
% \cmidrule{2-9}
% &\textbf{\ourmodel~+ BM25} & Hybrid & \textbf{71.3} & \textbf{83.6} & \textbf{80.0} & \textbf{85.4} & \textbf{69.1} & \textbf{80.9} \\
% \bottomrule
% \end{tabular}
% \caption{\amir{Not clear how this differs from table 1. Instead of "complementary", use the words I used for the other tables in the supp.} 
% Results complementary to Tables~\ref{tab:unsupervised} and \ref{tab:unsupervised_top100}. Top-20 and Top-100 retrieval accuracy on the \textit{original} test sets of NQ, TriviaQA and WQ for supervised and unsupervised approaches. DPR-Single is trained on the corresponding dataset only (except for EntityQs, where the model was trained on Natural Questions). DPR-Multi was trained on the first four datasets. We mark in bold the best unsupervised method for each dataset. }
% \label{tab:original_test_sets}
% \end{table*}

==> table_unsup_top100.tex <==

% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{cllcccccc}
% \toprule
% &\textbf{Model} & \textbf{Mode} & \textbf{NQ$^*$} & \textbf{TriviaQA$^*$} & \textbf{WQ$^*$} & \textbf{TREC} & \textbf{SQuAD} & \textbf{EntityQs}  \\
% % \midrule
% % \textit{Supervised Methods} & & & & & & &  \\
% \midrule
% \multirow{4.3}{55pt}{\textbf{\textit{Supervised}}} & DPR-Single & Dense  & 76.8 & 62.6 & 71.1 & 89.9 & 74.9 & 63.2 \\
% & DPR-Multi & Dense & 77.1 & 62.4 & 70.4 & 93.9 & 67.8 & 70.0 \\
% \cmidrule{2-9}
% & DPR-Single + BM25 & Hybrid & 81.1 & 64.9 & 72.8 & 93.8 & 86.3 & 81.3 \\
% & DPR-Mutli + BM25 & Hybrid & 80.9 & 65.2 & 73.0 & 95.4 & 83.0 & 82.6 \\
% \midrule
% % \textit{Unsupervised Methods} & & & & & & &  \\
% % \midrule
% \multirow{7}{55pt}{\textbf{\textit{Unsupervised}}}&BM25 & Sparse &  70.1 & 62.4 & 66.4 & 90.3 & 82.0 & 80.0 \\
% \cmidrule{2-9}
% % &ICT  & Dense & 51.3 & 14.2 & 52.1 & 35.2 & 27.3 & ~~4.8 \\
% &ICT  & Dense & 58.8 & 51.5 & 52.5 & - & 65.2 & - \\
% & Condenser & Dense &  26.6 & ~~9.1 & 30.8 & 34.4 & 25.3 & ~~7.6 \\
% & CoCondenser & Dense & 52.4 & 13.8 & 54.2 & 39.3 & 28.8 & ~~8.7 \\
% % &\textbf{\ourmodel} & Dense & 71.7 & 61.4 & 68.9 & 93.1 & 74.6 & 72.8 \\
% & \textbf{\ourmodel} & Dense & 72.8 & 61.9 & 69.3 & 92.7 & 75.2 & 74.4 \\
% \cmidrule{2-9}
% % &\textbf{\ourmodel~+ BM25} & Hybrid & \textbf{76.6} & \textbf{64.1} & \textbf{71.6} & \textbf{93.9} & \textbf{84.4} & \textbf{82.3} \\
% &\textbf{\ourmodel~+ BM25} & Hybrid & \textbf{77.3} & \textbf{64.3} & \textbf{71.5} & \textbf{93.5} & \textbf{84.4} & \textbf{82.2} \\
% \bottomrule
% \end{tabular}
% \caption{Results for an evaluation setup as in Table~\ref{tab:unsupervised} on additional datasets. Top-100 retrieval accuracy on the test sets of six datasets for supervised and unsupervised approaches. DPR-Single is trained on the corresponding dataset only (except for EntityQs, where the model was trained on Natural Questions, similar to \citealt{sciavolino-etal-2021-simple}). DPR-Multi was trained on the first four datasets. 
% We mark in bold the best unsupervised method for each dataset. 
% $^*$ For NQ, TriviaQA and WQ, we use the ``\textit{no answer overlap}'' potion of the test sets, to control for memorization issues which are not possible for unsupervised methods (see Section~\ref{sec:datasets}). Results on the original test sets are given in Table~\ref{tab:original_test_sets}.
% }
% \label{tab:unsupervised_top100}
% \end{table*}

